System-on-Chip Security Assertions

Assertions are widely used for functional validation as well as coverage analysis for both software and hardware designs. Assertions enable runtime error detection as well as faster localization of errors. While there is a vast literature on both software and hardware assertions for monitoring functional scenarios, there is limited effort in utilizing assertions to monitor System-on-Chip (SoC) security vulnerabilities. In this paper, we identify common SoC security vulnerabilities by analyzing the design. To monitor these vulnerabilities, we define several classes of assertions to enable runtime checking of security vulnerabilities. Our experimental results demonstrate that the security assertions generated by our proposed approach can detect all the inserted vulnerabilities while the functional assertions generated by state-of-the-art assertion generation techniques fail to detect most of them.

==> sections/assert_backup.tex <==
\section{Security Assertions}
To generate security assertions to detect the existence of the vulnerabilities 
outlined in Section~\ref{sec:vulner}, we use a combination of static (code) analysis and dynamic (execution trace) analysis, as shown in Figure~\ref{fig:classes}. This section mainly addresses two important questions: i) how to generate assertions automatically, and ii)
how to embed them in the design. The remainder of this section describes how to generate assertions as well as embedding them in RTL models.

\subsection{Embedding of Assertions} 
There are two orthogonal ways of embedding assertions in the RTL model of the SoC design: immediate and concurrent assertions. 
Please note that immediate assertions can be converted to concurrent assertions by modifying the antecedent. However, as described below, it would be natural
to use a specific one depending on the type of security vulnerability. 

\vspace{0.05in}
\noindent {\it Immediate Assertions:} Immediate assertions are powerful in detecting vulnerabilities such as permissions and privileges, and numeric errors. Immediate assertions are flexible and can vary based on the potential statements or blocks. For immediate operations, it is important to find out the exact location, the relevant variable (e.g., trigger) $\alpha$, and the assertion, {\it assert ($P(\alpha)$)}, can be inserted. Immediate assertions are inherent for checking specific operations, such as divide-by-zero checking, out-of-boundary checking.

\vspace{0.05in}
\noindent {\it Concurrent Assertions:} Concurrent assertions, on the other hand, are checked each clock cycle, representing expected properties of SoCs. Concurrent assertions are useful to express any FSM related vulnerabilities (e.g., illegal states and transitions). Each concurrent assertion can be defined using {\it assert property} $P$. The property $P$ should be derived from the specification of SoCs.

\subsection{Permissions and Privileges}
By reading the specification, we first find out the variable that represent the privilege level, e.g., CPSR in ARMv7. For each entry to a privileged operation block, we put an assertion to it. For the ease of illustration, we use \texttt{user} to represent current privilege, and \texttt{admin} to represent high privilege. Before privileged operation blocks, we are interested in the variable $\alpha : $ \texttt{user}, and define the property $P :$ \texttt{user == admin}, as shown in Listing~\ref{lst:privilege}.

\begin{lstlisting}[frame=single, caption={Permissions and Privileges}, language=Verilog, label={lst:privilege}]
always (@posedge clk) begin
    assert(user == admin);
    privileged operation block
end
\end{lstlisting}


\subsection{Resource Management}
Concurrent assertions are powerful in protecting resources from misusing in unexpected way. For example, to protect JTAG from using in normal operation mode, we add the assertion as shown in Listing~\ref{lst:resource}. 

\begin{lstlisting}[frame=single, caption={Resource Management}, language=Verilog, label={lst:resource}]
assert property (normal |-> !JTAG_enable);
\end{lstlisting}

\subsection{Undefined State/Transition}
The behaviors of SoCs are expressed in FSMs. As shown in Figure~\ref{fig:fsm}, circles represent states, and edges represent transitions between states. Listing~\ref{lst:state} gives an example of two assertions using SystemVerilog syntax \#\# to represent delay. The first assertion shows the correct transition and the second one shows the unexpected transition.

\begin{figure}[h]
    \centering
    \includegraphics{fig/fsm.eps}
    \caption{FSM example}
    \label{fig:fsm}
\end{figure}

\begin{lstlisting}[frame=single, caption={Undefined State/Transition}, language=Verilog, label={lst:state}]
assert property (A && a |=>  B);
assert property (!(C |=> A));
\end{lstlisting}

\subsection{Buffer Errors}
\label{subsub:buffer}
To prevent the index of buffer out of boundary, immediate assertions should be added before each buffer access. For example in Listing~\ref{lst:buffer}, before access \texttt{Buffer[index]}, we assert the variable $\alpha:$ \texttt{index} to satisfy property $P:$ \texttt{index >= 0 \&\& index <= limit}.

\begin{lstlisting}[frame=single, caption={Buffer Errors}, language=Verilog, label={lst:buffer}]
reg [limit:0] Buffer;
always (@posedge clk) begin
    assert(index >= 0 && index <= limit);
    access Buffer[index];
end
\end{lstlisting}

In addition, some properties may also require concurrent assertions to ensure global property. For example, to ensure the flush of instruction buffer (IB) after branch prediction failure, we use the assertion shown in Listing~\ref{lst:conbuffer}.

\begin{lstlisting}[frame=single, caption={Buffer Errors Concurrent Assertion}, language=Verilog, label={lst:conbuffer}]
assert property (Pre_fail |=> IB_Empty);
\end{lstlisting}

\subsection{Information Leakage}
To protect secret information from directly leaking to non-secure world, tagging is one potential solution. We assume that the results of secure world can only be passed to non-secure world through special interface (privileged instructions). For each normal operation consisting of both secure and non-secure variables, we need to check if the result is assigned to a non-secure variable. Assume $s$ is a secure variable in Listing~\ref{lst:information}. The operation of assigning the addition of $s$ and $a$ to $b$ needs to check the tag of $b$.

\begin{lstlisting}[frame=single, caption={Information Leakage}, language=Verilog, label={lst:information}]
reg s; // secure variable
reg a, b;   // two registers
reg s_t, a_t, b_t;  // tags
always (@posedge clk) begin
    ...
    assert(b_t == secure_tag);
    b = s + a;
    ...
end
\end{lstlisting}

\subsection{Numeric Errors}
Numeric errors are more relevant to the implementation of SoC designs. We use divide-by-zero as an example. After inspecting RTL implementation of SoC designs, we set $\alpha : $ \texttt{denominator}, and define the property $P :$ \texttt{denominator != 0}, as shown in Listing~\ref{lst:numeric}.

\begin{lstlisting}[frame=single, caption={Numeric Errors}, language=Verilog, label={lst:numeric}]
always (@posedge clk) begin
    assert(denominator != 0);
    quotient = numerator / denominator;
end
\end{lstlisting}

\subsection{Code Injection}
Hardware Trojans can be inserted during pre-silicon or post-silicon stage. In the pre-silicon stage, hardware Trojans are usually hidden in rare-to-activate branches. Assertions can be added in each rare branch to ensure the activation of rare branches during testing.

\begin{lstlisting}[frame=single, caption={Buffer Errors}, language=Verilog, label={lst:buffer}]
reg [128:0] trigger;
always (@posedge clk) begin
    if (trigger == 0) begin
        assert(true);
        ...
    end
end
\end{lstlisting}


==> sections/case_backup.tex <==
\section{Case Study}
\label{sec:case}

To demonstrate the necessity of security assertions, we analyzed four benchmarks and inserted potential security assertions introduced in Section~\ref{sec:assert}. Then, Goldmine \cite{Hertz:2013} was applied to all these benchmarks to generate as many assertions as possible. Finally, we simulated the design with directed test to activate our assertions. For each of our assertion, Goldmine is claimed to catch the corresponding vulnerability if the assertions generated by Goldmine also raise a flag during simulation. The summary of potential vulnerabilities of each benchmarks is shown in Table~\ref{tab:result}. In the remainder of this section, we will explain each vulnerability in detail.

% \begin{figure}[h]
%     \centering
%     \includegraphics{fig/experiment.eps}
%     \caption{Experimental Setup}
%     \label{fig:experiment}
% \end{figure}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        Vulnerability & Arbiter & MEM & GNG & AES\\
        \hline
        Permissions and Privileges & & \checkmark  & & \\
        \hline
        Resource Management & & & & \checkmark \\
        \hline
        Illegal States \& Transitions & \checkmark/\checkmark & \checkmark & &\\
        \hline
        Buffer Issues & & \checkmark & &\\
        \hline
        Information Leakage & \checkmark/\checkmark & & &\\
        \hline
        Numeric Exceptions & & & \checkmark &\\
        \hline
        Malicious Implants & & & & \checkmark\\
        \hline
    \end{tabular}
    \caption{The types of vulnerabilities in four designs. Note that more potential vulnerabilities are possible in all designs. We select these types for illustration.}
    \label{tab:result}
\end{table}

\subsection{Arbiter}
We first analyzed a simple design, Arbiter, as shown in Listing~\ref{lst:arbiter}. This design consists of four input signals and two output signals, including clk and rst. For this simple design, most of the vulnerabilities listed in Section~\ref{sec:vulner} do not exist, e.g., permission and privileges, buffer errors, and so on. We identified the following two potential vulnerabilities:
\begin{enumerate}
    \item Invalid states and transitions. While functional test focuses on valid states and transitions, security assertions are mainly about invalid or unstated transitions. One simple assertion is checking gnt1 and gnt2 are never asserted together, i.e., assert(!(gnt1 \& gnt2)). Although this assertion will be never asserted during normal usage, runtime checking can detect errors such as fault injection and transient errors. However, the number of invalid states and transitions are infinite. For example, when we consider two consecutive cycles, assert(!(gnt1 $|=>$ (gnt2 != req2))) should hold. 
    \item Information leakage. Assume that req1 is connected to some key-related variable. We do not want any output signal to be always the same as req1, i.e., assert(!G(gnt1 == req1)) and assert(!G(gnt2 == req1)). When the req2 is randomly given, there exists some point when gnt1 is not equal to req1. The same argument holds for gnt2. 
\end{enumerate}

\begin{lstlisting}[frame=single, caption={Arbiter}, language=Verilog, label={lst:arbiter}]
module arb2(clk, rst, req1, 
            req2, gnt1, gnt2);
  
input clk, rst;
input req1, req2;
output gnt1, gnt2;

reg state;
reg gnt1, gnt2;

always @ (posedge clk or posedge rst)
    if (rst)
        state <= 0;
    else
        state <= gnt1;

always @ (*)
    if (state)
    begin
        gnt1 = req1 & ~req2;
        gnt2 = req2;
    end
    else
    begin
        gnt1 = req1;
        gnt2 = req2 & ~req1;
    end

endmodule
\end{lstlisting}

The assertions generated by goldmine are shown in Listing~\ref{lst:assertions}. As goldmine analyzes the golden design shown in Listing~\ref{lst:arbiter} by mining the traces of random simulation, it is able to capture reachable states and transitions. It can be verified that these assertions cover all the valid transitions for this small design. Since the two assertions of our approach is directly relevant to the FSM and contain only the input and output signals, Goldmine is able to capture all the vulnerabilities analyzed above.

\begin{lstlisting}[frame=single, caption={Assertions by Goldmine}, language=Verilog, label={lst:assertions}]
(state == 1 & req2 == 1) |-> (gnt1 == 0)
(req1 == 1 & state == 0) |-> (gnt1 == 1)
(req1 == 0) |-> (gnt1 == 0)
(req1 == 1 & req2 == 0) |-> (gnt1 == 1)

(req1 == 1 & state == 0) |-> (gnt2 == 0)
(req2 == 1 & state == 1) |-> (gnt2 == 1)
(req2 == 0) |-> (gnt2 == 0)
(req2 == 1 & req1 == 0) |-> (gnt2 == 1)
\end{lstlisting}




\subsection{A Simplified Memory Design}
The second design is created to mimic the behavior of a simplified Trusted Hardware (TH) implementation of its memory, as shown in Listing~\ref{lst:memory}. Trusted Hardware, e.g., Intel’s Software Guard Extensions (SGX) \cite{sgx}, allows remote clients to upload private computation and data to a secure container of a server with a TH. One key implementation of SGX is the introduction of Process Reserved Memory and Enclave Page Cache (EPC), inhibiting invalid accesses even from the kernel.

The simplified design in Listing~\ref{lst:memory} contains five input singals (clk, rst, wr to denote write if asserted, sc to denote whether it is a secure access or not, address, and in to denote the value to write) and one output signal (out to denote the output of read). The memory space is denoted by an array named mem with size of 12GB.

\begin{enumerate}
    \item Permissions and Privileges. Assume the lower 1kB of memory is allocated to EPC. Since EPC should be access through secure container/process, each access to the lower 1kB should be checked. Although one conditional checking is already in place, assertions may also help when implementation error, fault injection or Hardware Trojans exist. For example, assert(address $<=$ 1024 $|=>$ sc) can be inserted before two accesses.
    \item Undefined state/transition. In this simplified memory implementation, it does not explicitly describe the state of out signal when we want to write. For a buggy CPU design which connects to this memory, a process will be able to read the previous access of another process from the out port (including secure processes) with interleaved memory access. We need add a concurrent assertion with (assert property (wr $|=>$ out == 0));
    \item Buffer errors. Memory as one type of buffer should be checked for buffer errors. Therefore, each access to memory should be checked with assertions to test if address is in the range of memory size. In this example, the memory size is 12GB ($3 * 2^{32}$) and the length of address is 34 bits. Therefore, we need to test if the address is within the size of memory, assert(address $< 3* 2**32$).
\end{enumerate}

\begin{lstlisting}[frame=single, caption={Simplified Memory of Trusted Hardware}, language=Verilog, label={lst:memory}]
module mem(clk, rst, wr, sc, address,
            in, out);
  
input clk, rst, wr, sc;
input [33:0]address;
input [7:0]in;
output reg [7:0]out;

reg[7:0] mem[3* 2**32-1:0];
reg[33:0] i;

initial begin
    for (i = 0; i < 3* 2**32 - 1;
        i = i + 1) begin
        mem[i] <= 0;
    end
end

always @ (posedge clk) begin
    if (address >= 1024 || sc) begin
        if (wr) begin
            mem[address] <= in;
        end
        else begin
            out <= mem[address];
        end
    end
end

endmodule
\end{lstlisting}

However, goldmine did not generate any assertions. However, as it fail to see the implementation details of the design, it is impossible for Goldmine to generate assertions for vulnerabilities such as numeric errors and code injections.


% To show that the assertions generated by goldmine do not cover the security vulnerabilities, we appended the four assertions generated by goldmine to the end of the vulnerable version in Listing~\ref{lst:vulner} and simulated using ModelSim. Directed tested are used to activated the vulnerabilities. From the simulation, we observed that none of the assertions are triggered although these vulnerabilities are activated by these directed tests.


\subsection{Gaussian Noise Generator (GNG)}
To show numeric errors in real design, we next inspect a computation-intense design called Gaussian Noise Generator (GNG). The design is downloaded from opencores \cite{OpenCores}. Instead of delving into the details of Gaussian Noise Generating algorithms, we inspect the RTL design as a normal program and generate general security assertions for it. 

One possible numeric error in this design is the assignments between signed and unsigned values as shown in the snippet of code in Listing~\ref{lst:gng}. The first assignment assigns an unsigned variable to a signed variable. Next assignment is the computation between signed values. The final assignment assigns a signed value to an unsigned value. Without knowing the intention of this code, we are concerned with the automatic tranformation between signed and unsigned values. For example, when the $32^{th}$ bit of mul1 is 1, mul1\_new is interpreted as a negative value using a two's complement representation. Then mul\_new is added to a positive number and converted to an unsigned number again. The behavior may not be the original intention of this code. We want to generate assertions, e.g., assert(mul1[32] != 1), and let the user decide if it is a numeric error or the expected behavior.  

\begin{lstlisting}[frame=single, caption={GNG\_interp}, language=Verilog, label={lst:gng}]
module gng_interp (
    input clk, 
    input rstn, 

    // Data interface
    input valid_in,
    input [63:0] data_in,
    output reg valid_out, 
    output reg [15:0] data_out
);
  
wire [33:0] mul1;
wire signed [13:0] mul1_new;
reg [17:0] c0_r5;
reg signed [18:0] sum2;
reg [14:0] sum2_rnd;

...

assign mul1_new = mul1[32:19];

always @ (posedge clk) begin
    sum2 <= $signed({1'b0, c0_r5}) + 
        mul1_new;
end

always @ (posedge clk) begin
    sum2_rnd <= sum2[17:3] + sum2[2];
end

...

endmodule
\end{lstlisting}

\subsection{AES}
Advanced Encryption Standard (AES) is a very commonly used crypto core. AES consists of ten rounds of block ciphers which is a substitution permutation network. The substitution part of code is shown in Listing~\ref{lst:aes}. As module S contains a lot of rare branches, attackers tend to insert Hardware Trojans based on these rare branches. For example, assert(out != 32'h7c7c7c7c) in module S4 can be used to check if (in == 8'h01) is true in S\_0, S\_1, S\_2 and S\_3 all together. The probability of this trigger is $2^{-32}$. However, the total number different combinations is $2^{32}$, making it infeasible to insert all such assertions. The problem of assertions refinement is beyond the scope of this paper.


\begin{lstlisting}[frame=single, caption={AES table}, language=Verilog, label={lst:aes}]
/* substitue four bytes in a word */                                   
module S4 (clk, JTAG, in, out);
    input clk, JTAG;
    input [31:0] in;
    output [31:0] out;
    S
        S_0 (clk, in[31:24], out[31:24]),
        S_1 (clk, in[23:16], out[23:16]),
        S_2 (clk, in[15:8],  out[15:8] ),
        S_3 (clk, in[7:0],   out[7:0]  );
    
    always @ (posedge clk)
    if (JTAG)
        $display(in);
    endcase
endmodule

module S (clk, in, out);
    input clk;
    input [7:0] in;
    output reg [7:0] out;
    
    always @ (posedge clk)
    case (in)
        8'h00: out <= 8'h63;
        8'h01: out <= 8'h7c;
        ...
    endcase
endmodule
\end{lstlisting}



==> sections/property.tex <==
\section{Model Checking}
The vulnerabilities can also be used to generate properties for model checking.

==> sections/reference.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{foster2004assertion}
H.~D. Foster, A.~C. Krolnik, and D.~J. Lacey, \emph{Assertion-based
  design}.\hskip 1em plus 0.5em minus 0.4em\relax Springer Science \& Business
  Media, 2004.

\bibitem{Ray:2018}
S. Ray et al., ``System-on-Chip Platform Security Assurance: Architecture and Validation,'' in \emph{Proceedings of the IEEE}, 2018.

% \bibitem{farahmandi2017cost}
% F.~Farahmandi, R.~Morad, A.~Ziv, Z.~Nevo, and P.~Mishra, ``Cost-effective
%   analysis of post-silicon functional coverage events,'' in \emph{DATE}, 2017.

\bibitem{TrustHub}
``Trusthub,'' \url{https://www.trust-hub.org}.

\bibitem{cwe}
``Common weakness enumeration,'' \url{https://cwe.mitre.org}.

\bibitem{nvd}
``National vulnerability database,'' https://nvd.nist.gov.

% \bibitem{Edmund:1982}
% E.~M. Clarke and E.~A. Emerson, ``Design and synthesis of synchronization
%   skeletons using branching time temporal logic,'' in \emph{Logics of
%   Programs}, 1982.

\bibitem{di2013integration}
G.~Di~Guglielmo et al., ``On the integration of model-driven design
  and dynamic assertion-based verification for embedded software,''
  \emph{Journal of Systems and Software}, 2013.

\bibitem{ieee2010psl}
``{1850-2010 - IEEE Standard for Property Specification Language (PSL)},''
  2010.

\bibitem{ieee2012sva}
``{1800-2012 - IEEE Standard for SystemVerilog--Unified Hardware Design,
  Specification, and Verification Language},'' 2012.

\bibitem{ben1983temporal}
M.~Ben-Ari, A.~Pnueli, and Z.~Manna, ``The temporal logic of branching time,''
  \emph{Acta informatica}, 1983.

\bibitem{armoni2002forspec}
R.~Armoni et al., ``The forspec
  temporal logic: A new temporal property-specification language,'' in
  \emph{TACAS}, 2002.

\bibitem{bauer2011theory}
A.~Bauer and M.~Leucker, ``The theory and practice of salt,'' in \emph{NASA
  Formal Methods Symposium}, 2011.

\bibitem{tabakov2008temporal}
D.~Tabakov, G.~Kamhi, M.~Y. Vardi, and E.~Singerman, ``A temporal language for
  systemc,'' in \emph{FMCAD}, 2008.

\bibitem{foster2006introduction}
H.~Foster, K.~Larsen, and M.~Turpin, ``Introduction to the new accellera open
  verification library,'' in \emph{DVCon}, 2006.

\bibitem{Rogin:2008}
F.~Rogin et al., ``Automatic generation
  of complex properties for hardware designs,'' in \emph{DATE}, 2008.

\bibitem{Hertz:2013}
S.~Hertz, D.~Sheridan, and S.~Vasudevan, ``Mining hardware assertions with
  guidance from static analysis,'' \emph{TCAD}, 2013.

\bibitem{Wang:2018}
C.~{Wang} et al.,
``Asax: Automatic security assertion extraction for detecting hardware
  trojans,''
\newblock In {\em ASP-DAC}, 2018.

\bibitem{trustzone}
``Arm trustzone,'' https://developer.arm.com/technologies/trustzone.

\bibitem{OpenCores}
``Opencores,'' \url{https://www.opencores.org}.

\bibitem{sgx}
``Intel® software guard extensions,'' https://software.intel.com/en-us/sgx.

\end{thebibliography}
